Multi-Resolution Weak Supervision for Sequential Data

Since manually labeling training data is slow and expensive, recent industrial and scientific research efforts have turned to weaker or noisier forms of supervision sources. However, existing weak supervision approaches fail to model multi-resolution sources for sequential data, like video, that can assign labels to individual elements or collections of elements in a sequence. A key challenge in weak supervision is estimating the unknown accuracies and correlations of these sources without using labeled data. Multi-resolution sources exacerbate this challenge due to complex correlations and sample complexity that scales in the length of the sequence. We propose Dugong, the first framework to model multi-resolution weak supervision sources with complex correlations to assign probabilistic labels to training data. Theoretically, we prove that Dugong, under mild conditions, can uniquely recover the unobserved accuracy and correlation parameters and use parameter sharing to improve sample complexity. Our method assigns clinician-validated labels to population-scale biomedical video repositories, helping outperform traditional supervision by 36.8 F1 points and addressing a key use case where machine learning has been severely limited by the lack of expert labeled data. On average, Dugong improves over traditional supervision by 16.0 F1 points and existing weak supervision approaches by 24.2 F1 points across several video and sensor classification tasks.

==> tables/ablation_table.tex <==
%!TEX root = ../neurips_2019.tex

\begin{table}[]
    \centering
    \begin{tabular}{@{}lccccc@{}}
        \toprule
                                             & \multicolumn{2}{c}{\textbf{Parameter Ablation}} & \multicolumn{3}{c}{\textbf{Class Prior}}                                    \\ \cmidrule(l){2-3} \cmidrule(l){4-6}
        \textbf{Dataset} & \textbf{w.o Param Red.} & \textbf{w.o Temp Deps} & \textbf{Uniform}        & \textbf{Dev}            & \textbf{User}           \\ \midrule        BAV                                  & 36.3 $\pm$ 2.7         & 50.1 $\pm$5.4          & 4.7 $\pm$ 3.9           & 53.2 $\pm$ 2.2 & \textbf{58.9 $\pm$ 2.2}          \\
        Open                                 & 62.1 $\pm$ 3.7         & 60.6 $\pm$ 2.9         & 62.6 $\pm$ 7.0          & 68.8 $\pm$ 3.2          & \textbf{70.5 $\pm$ 4.8} \\
        Gait                                 & 59.5 $\pm$ 5.4         & 65.3 $\pm$ 2.2         & \textbf{68.0 $\pm$ 0.7} & 67.2 $\pm$ 0.6          & 66.4 $\pm$ 1.1          \\
        Shot                                 & 86.6 $\pm$ 1.3         & 86.6 $\pm$ 0.5         & 72.9 $\pm$ 3.4          & 81.1 $\pm$ 1.2          & \textbf{87.7 $\pm$ 1.0} \\ 
        Basketball                          & 32.9 $\pm$ 4.9         & 9.9 $\pm$ 0.8          & 18.3 $\pm$ 0.0          & 27.6 $\pm$ 15.4          & \textbf{38.2 $\pm$ 4.1} \\ \bottomrule
        \end{tabular}
    \caption{End model performance of ablation studies in terms of F1 score (mean $\pm$ std.dev). Bolded entries represent the best performance using label from our model. Incorporating temporal dependencies and parameter sharing helps performance significantly while the advantage of setting the class prior manually is task-specific. \todo{might move part to appendix if space constrained}}
    \label{table:ablation}
\end{table}

==> tables/supervision_sources.tex <==
%!TEX root = ../neurips_2019.tex


\begin{table}[ht!]
    \centering
    \small
    \begin{tabular}{@{}lccccccccc@{}}
        \toprule
        \textbf{Name}    & \textbf{Weak Supervision Source} & \textbf{Description}  \\ \cmidrule(l){1-3}
        \texttt{}        & \texttt{}                        &                       \\
        \texttt{}        & \texttt{}                        &                       \\
        \texttt{}        & \texttt{}                        &                       \\
        \texttt{}        & \texttt{}                        &                       \\
        \texttt{}        & \texttt{}                        &                       \\ \bottomrule
        \end{tabular}
    \caption{Weak Supervision Sources for the BAV task.}
    \label{table:ws_BAV}
\end{table}

\begin{table}[ht!]
    \centering
    \small
    \begin{tabular}{@{}lccccccccc@{}}
        \toprule
        \textbf{Name}    & \textbf{Weak Supervision Source} & \textbf{Description}  \\ \cmidrule(l){1-3}
        \texttt{}        & \texttt{}                        &                       \\
        \texttt{}        & \texttt{}                        &                       \\
        \texttt{}        & \texttt{}                        &                       \\
        \texttt{}        & \texttt{}                        &                       \\
        \texttt{}        & \texttt{}                        &                       \\ \bottomrule
        \end{tabular}
    \caption{Weak Supervision Sources for the BAV task.}
    \label{table:ws_BAV}
\end{table}

\begin{table}[ht!]
    \centering
    \small
    \begin{tabular}{@{}lccccccccc@{}}
        \toprule
        \textbf{Name}    & \textbf{Weak Supervision Source} & \textbf{Description}  \\ \cmidrule(l){1-3}
        \texttt{}        & \texttt{}                        &                       \\
        \texttt{}        & \texttt{}                        &                       \\
        \texttt{}        & \texttt{}                        &                       \\
        \texttt{}        & \texttt{}                        &                       \\
        \texttt{}        & \texttt{}                        &                       \\ \bottomrule
        \end{tabular}
    \caption{Weak Supervision Sources for the Open task.}
    \label{table:ws_open}
\end{table}

\begin{table}[ht!]
    \centering
    \small
    \begin{tabular}{@{}lccccccccc@{}}
        \toprule
        \textbf{Name}    & \textbf{Weak Supervision Source} & \textbf{Description}  \\ \cmidrule(l){1-3}
        \texttt{}        & \texttt{}                        &                       \\
        \texttt{}        & \texttt{}                        &                       \\
        \texttt{}        & \texttt{}                        &                       \\
        \texttt{}        & \texttt{}                        &                       \\
        \texttt{}        & \texttt{}                        &                       \\ \bottomrule
        \end{tabular}
    \caption{Weak Supervision Sources for the Gait task.}
    \label{table:ws_gait}
\end{table}

\begin{table}[ht!]
    \centering
    \small
    \begin{tabular}{@{}lll@{}}
        \toprule
        \textbf{Name}                & \textbf{Weak Supervision Source}                               & \textbf{Description}               \\ \cmidrule(l){1-3}
        \texttt{ws\_hsv}             & \texttt{diffs = [hsvhists[i] - hsvhists[i-1]]};                & Detect a shot change if there's an \\
                                     & 1 if \texttt{diffs[i] - mean(diffs[i-500:i+500])} $\geq$       & outlier in HSV histogram changes   \\
                                     & ~~~~\texttt{2.5 * stddev(diffs[i-500:i+500])};                 & between frames                     \\
                                     & -1 if \texttt{diffs[i] - mean(diffs[i-500:i+500])} $\leq$      &                                    \\
                                     & ~~~~\texttt{1.0 * stddev(diffs[i-500:i+500])};                 &                                    \\
                                     & 0 otherwise                                                    &                                    \\
        \texttt{ws\_rgb}             & \texttt{diffs = [rgbhists[i] - rgbhists[i-1]]};                & Detect a shot change if there's an \\
                                     & 1 if \texttt{diffs[i] - mean(diffs[i-500:i+500])} $\geq$       & outlier in RGB histogram changes   \\
                                     & ~~~~\texttt{2.5 * stddev(diffs[i-500:i+500])};                 & between frames                     \\
                                     & -1 if \texttt{diffs[i] - mean(diffs[i-500:i+500])} $\leq$      &                                    \\
                                     & ~~~~\texttt{1.0 * stddev(diffs[i-500:i+500])};                 &                                    \\
                                     & 0 otherwise                                                    &                                    \\
        \texttt{ws\_flow}            & \texttt{diffs = [flowhists[i] - flowhists[i-1]]};              & Detect a shot change if there's an \\
                                     & 1 if \texttt{diffs[i] - mean(diffs[i-500:i+500])} $\geq$       & outlier in optical flow histogram  \\
                                     & ~~~~\texttt{2.5 * stddev(diffs[i-500:i+500])};                 & changes  between frames            \\
                                     & -1 if \texttt{diffs[i] - mean(diffs[i-500:i+500])} $\leq$      &                                    \\
                                     & ~~~~\texttt{1.0 * stddev(diffs[i-500:i+500])};                 &                                    \\
                                     & 0 otherwise                                                    &                                    \\
        \texttt{ws\_face\_counts}    & -1 if \texttt{len(faces[seq\_end]) ==}                         & Say there is no shot change if the \\
                                     & ~~~~\texttt{len(faces[seq\_start])};                           & number of faces stays the same     \\
                                     & 0 otherwise                                                    &                                    \\
        \texttt{ws\_face\_positions} & 1 if \texttt{positions\_match(}                                & Say there is a shot change if the  \\
                                     & ~~~~\texttt{faces[seq\_end], faces[seq\_start])};              & faces change position, no shot     \\
                                     & -1 if \texttt{positions\_change(}                              & change if the faces stay in the    \\
                                     & ~~~~\texttt{faces[seq\_end], faces[seq\_start])};              & same place, abstain if no faces    \\
                                     & 0 otherwise                                                    & detected                           \\ \bottomrule
        \end{tabular}
    \caption{Weak Supervision Sources for the shot task.}
    \label{table:ws_shot}
\end{table}

\begin{table}[ht!]
    \centering
    \small
    \begin{tabular}{@{}lccccccccc@{}}
        \toprule
        \textbf{Name}    & \textbf{Weak Supervision Source} & \textbf{Description}  \\ \cmidrule(l){1-3}
        \texttt{}        & \texttt{}                        &                       \\
        \texttt{}        & \texttt{}                        &                       \\
        \texttt{}        & \texttt{}                        &                       \\
        \texttt{}        & \texttt{}                        &                       \\
        \texttt{}        & \texttt{}                        &                       \\ \bottomrule
        \end{tabular}
    \caption{Weak Supervision Sources for the basketball task.}
    \label{table:ws_basketball}
\end{table}

